EnergyMatch: Energy-based Pseudo-Labeling for Semi-Supervised Learning

Recent state-of-the-art methods in semi-supervised learning (SSL) combine consistency regularization with confidence-based pseudo-labeling. To obtain high-quality pseudo-labels, a high confidence threshold is typically adopted. However, it has been shown that softmax-based confidence scores in deep networks can be arbitrarily high for samples far from the training data, and thus, the pseudo-labels for even high-confidence unlabeled samples may still be unreliable. In this work, we present a new perspective of pseudo-labeling: instead of relying on model confidence, we instead measure whether an unlabeled sample is likely to be "in-distribution"; i.e., close to the current training data. To classify whether an unlabeled sample is "in-distribution" or "out-of-distribution", we adopt the energy score from out-of-distribution detection literature. As training progresses and more unlabeled samples become in-distribution and contribute to training, the combined labeled and pseudo-labeled data can better approximate the true distribution to improve the model. Experiments demonstrate that our energy-based pseudo-labeling method, albeit conceptually simple, significantly outperforms confidence-based methods on imbalanced SSL benchmarks, and achieves competitive performance on class-balanced data. For example, it produces a 4-6% absolute accuracy improvement on CIFAR10-LT when the imbalance ratio is higher than 50. When combined with state-of-the-art long-tailed SSL methods, further improvements are attained.

==> figures/visualization.tex <==
\begin{figure}[t]
\centering
\subfloat[Energy-based Pseudo-label Decision]{%
  \includegraphics[width=\linewidth]{pics/energy_vis.pdf}%
  \label{fig:cifar_thres}%
}\qquad
\subfloat[Confidence-based Pseudo-label Decision]{%
  \includegraphics[width=\linewidth]{pics/confidence_vis.pdf}%
  \label{fig:cifar_lt_thres}%
}\qquad
\caption{\textbf{Visualization: energy score vs confidence score}: The shaded region denotes the which data points are pseudo-labeled. (a) Energy-based Pseudo-Label Decision and (b) Confidence-based Pseudo-Label Decision. Notice that energy-based pseudo-labelling produces correct pseudo-labels for many low-confident unlabeled examples.}
\label{fig:visualization}
\end{figure}

==> sections/border.tex <==
\section*{Broader Impact}
In this work, we propose energy-based pseudo-labelling in replacement of the vanilla confidence-based pseudo-labelling for semi-supervised learning. Our method is simple and achieves promising performance with both balanced and imbalanced data, which makes the deployment of semi-supervised learning more plausible in real-world scenarios. Ideally, our method could help with real world scenarios with positive applications such as reducing human annotation effort in medical image understanding though misuse for the negative applications such as surveillance is also possible. This would be a potential social impact of any advances of label-efficient learning methods, which we hope would never happen.
